FINECAPTION: Compositional Image Captioning Focusing on Wherever You Want at Any Granularity

The advent of large Vision-Language Models (VLMs) has significantly advanced multimodal tasks, enabling more sophisticated and accurate reasoning across various applications, including image and video captioning, visual question answering, and cross-modal retrieval. Despite their superior capabilities, VLMs struggle with fine-grained image regional composition information perception. Specifically, they have difficulty accurately aligning the segmentation masks with the corresponding semantics and precisely describing the compositional aspects of the referred regions. However, compositionality - the ability to understand and generate novel combinations of known visual and textual components - is critical for facilitating coherent reasoning and understanding across modalities by VLMs. To address this issue, we propose FINECAPTION, a novel VLM that can recognize arbitrary masks as referential inputs and process high-resolution images for compositional image captioning at different granularity levels. To support this endeavor, we introduce COMPOSITIONCAP, a new dataset for multi-grained region compositional image captioning, which introduces the task of compositional attribute-aware regional image captioning. Empirical results demonstrate the effectiveness of our proposed model compared to other state-of-the-art VLMs. Additionally, we analyze the capabilities of current VLMs in recognizing various visual prompts for compositional region image captioning, highlighting areas for improvement in VLM design and training.

==> preamble.tex <==
%
% --- inline annotations
%

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\definecolor{SP}{RGB}{114, 97, 171}

==> sec/limitation.tex <==
\section{Limitation and Future Work}


==> tables/aspects_explain.tex <==
\begin{table*}[htbp]
\centering
\caption{Descriptions of Various Categories}
\begin{tabular}{ll}
\toprule
\textbf{Category} & \textbf{Description} \\
\midrule
\textbf{Category Name} & The specific label or name of the category being described. \\
\textbf{Body Shape} & The general shape or silhouette of the body (e.g., slim, bulky). \\
\textbf{Skin Texture and Color} & Describes the texture (e.g., smooth, rough) and color of the skin. \\
\textbf{Clothing, Shoes, Accessories} & Describes clothing, footwear, and accessories worn by the subject. \\
\textbf{Interaction with Other Objects} & How the subject interacts with other objects (e.g., holding, sitting on). \\
\textbf{Body Pose/Gesture} & The posture or gestures of the body (e.g., standing, waving). \\
\textbf{More Description} & Additional descriptive elements not covered by other categories. \\
\textbf{Relative Location with Other Objects} & The spatial relationship between the subject and other objects. \\
\textbf{Color} & The color(s) associated with the subject or objects. \\
\textbf{Materials/Texture} & Describes the materials or texture of objects or surfaces (e.g., metal, soft). \\
\textbf{Camera Viewpoint} & The perspective or angle from which the image is captured (e.g., top view, side view). \\
\textbf{Associative Visual Effect} & Visual effects that are associated with the object (e.g., shadows, reflections). \\
\textbf{Shape} & The shape or form of the object or subject. \\
\textbf{Facial Expression} & Describes the expression on the face (e.g., smiling, frowning). \\
\textbf{Hair} & Details about hair, such as style, color, and texture. \\
\textbf{Age Ranging} & An estimation or description of the age range of the subject. \\
\textbf{Object Pose for Deformable Object} & The shape or posture of flexible objects (e.g., fabric, paper). \\
\textbf{Style} & Describes the style or fashion associated with the subject or object. \\
\bottomrule
\end{tabular}
\end{table*}
